Carina: Interactive Million-Node Graph Visualization using Web Browser Technologies

We are working on a scalable, interactive visualization system, called Carina, for people to explore million-node graphs. By using latest web browser technologies, Carina offers fast graph rendering via WebGL, and works across desktop (via Electron) and mobile platforms. Different from most existing graph visualization tools, Carina does not store the full graph in RAM, enabling it to work with graphs with up to 69M edges. We are working to improve and open-source Carina, to offer researchers and practitioners a new, scalable way to explore and visualize large graph datasets.

==> Makefile <==
### latex.makefile
# Author: Jason Hiebel

# This is a simple makefile for compiling LaTeX documents. The core assumption
# is that the resulting documents should have any parameters effecting
# rendering quality set to theoretical limits and that all fonts should be
# embedded. While typically overkill, the detriment to doing so is negligible.

# Targets:
#    default : compiles the document to a PDF file using the defined
#              latex generating engine. (pdflatex, xelatex, etc)
#    display : displays the compiled document in a common PDF viewer.
#              (currently linux = evince, OSX = open)
#    clean   : removes the obj/ directory holding temporary files
PROJECT = carina
default: obj/$(PROJECT).pdf

display: default
	(${PDFVIEWER} obj/$(PROJECT).pdf &)


### Compilation Flags
PDFLATEX_FLAGS  = -halt-on-error -output-directory obj/

TEXINPUTS = .:obj/
TEXMFOUTPUT = obj/


### File Types (for dependancies)
TEX_FILES = $(shell find . -name '*.tex' -or -name '*.sty' -or -name '*.cls')
BIB_FILES = $(shell find . -name '*.bib')
BST_FILES = $(shell find . -name '*.bst')
IMG_FILES = $(shell find . -path '*.jpg' -or -path '*.png' -or \( \! -path './obj/*.pdf' -path '*.pdf' \) )


### Standard PDF Viewers
# Defines a set of standard PDF viewer tools to use when displaying the result
# with the display target. Currently chosen are defaults which should work on
# most linux systems with GNOME installed and on all OSX systems.

UNAME := $(shell uname)

ifeq ($(UNAME), Linux)
PDFVIEWER = evince
endif

ifeq ($(UNAME), Darwin)
PDFVIEWER = open
endif


### Clean
# This target cleans the temporary files generated by the tex programs in
# use. All temporary files generated by this makefile will be placed in obj/
# so cleanup is easy.

clean::
	rm -rf obj/

### Core Latex Generation
# Performs the typical build process for latex generations so that all
# references are resolved correctly. If adding components to this run-time
# always take caution and implement the worst case set of commands.
# Example: latex, bibtex, latex, latex
#
# Note the use of order-only prerequisites (prerequisites following the |).
# Order-only prerequisites do not effect the target -- if the order-only
# prerequisite has changed and none of the normal prerequisites have changed
# then this target IS NOT run.
#
# In order to function for projects which use a subset of the provided features
# it is important to verify that optional dependancies exist before calling a
# target; for instance, see how bibliography files (.bbl) are handled as a
# dependency.

obj/:
	mkdir -p obj/

obj/$(PROJECT).aux: $(TEX_FILES) $(IMG_FILES) | obj/
	xelatex $(PDFLATEX_FLAGS) $(PROJECT)

obj/$(PROJECT).bbl: $(BIB_FILES) | obj/$(PROJECT).aux
	bibtex obj/$(PROJECT)
	xelatex $(PDFLATEX_FLAGS) $(PROJECT)

obj/$(PROJECT).pdf: obj/$(PROJECT).aux $(if $(BIB_FILES), obj/$(PROJECT).bbl)
	xelatex $(PDFLATEX_FLAGS) $(PROJECT)

